VALSE: A Task-Independent Benchmark for Vision and Language Models Centered on Linguistic Phenomena

We propose VALSE (Vision And Language Structured Evaluation), a novel benchmark designed for testing general-purpose pretrained vision and language (V&L) models for their visio-linguistic grounding capabilities on specific linguistic phenomena. VALSE offers a suite of six tests covering various linguistic constructs. Solving these requires models to ground linguistic phenomena in the visual modality, allowing more fine-grained evaluations than hitherto possible. We build VALSE using methods that support the construction of valid foils, and report results from evaluating five widely-used V&L models. Our experiments suggest that current models have considerable difficulty addressing most phenomena. Hence, we expect VALSE to serve as an important benchmark to measure future progress of pretrained V&L models from a linguistic perspective, complementing the canonical task-centred V&L evaluations.

==> tables/bench_results2.tex <==

\begin{table*}[t!]
    \centering
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{@{}l c | c | c  c | c c c c c }
        \toprule
         & & & \multicolumn{2}{c|}{Unimodal} & \multicolumn{5}{c}{Multimodal zero-shot}\\
        \bf Phenomenon & \bf Metric & \bf Rand. & \bf GPT1 & \bf GPT2 & \bf CLIP & \bf LXMERT & \bf ViLBERT & \bf ViLBERT 12-in-1 & \bf VisualBERT\\
        \midrule
        \multirow{4}{*}{Existence} & $acc$ & 50.0 & -- & -- & -- & 55.8 & 2.4 & 89.0 & \\
         & $p_c$ & 50.0 & -- & -- & -- & 41.6 & 56.8 & 85.0 &\\ 
         & $p_f$ & 50.0 & -- & -- & -- & 70.1 &	47.9 &93.1 & \\ 
         & $acc_r$ & 50.0 & 61.8 &	58.0 &	66.9 & 78.6 & 65.5 & 95.6 & \\
        \midrule
        \multirow{4}{*}{\parbox{17mm}{Plurality}} & $acc$ & 50.0 & -- & -- & -- & 55.1 & 50.3 & 62.0 & \\
         & $p_c$ & 50.0 & -- & -- & -- &  68.0 & 98.5 & 90.7\\ 
         & $p_f$ & 50.0 & -- & -- & -- & 42.2 & 2.1 & 33.4 & \\ 
         & $acc_r$ & 50.0 & 53.1 & 51.9  & 56.2 & 64.4 & 61.2 & 72.4 &  \\
        \midrule
         \multirow{4}{*}{\parbox{17mm}{Counting}} & $acc$ & 50.0 & -- & -- & -- & 52.0 & 50.7 & 64.9  & \\
         & $p_c$ & 50.0 & -- & -- & -- &  50.9 & 77.0 & 64.3\\ 
         & $p_f$ & 50.0 & -- & -- & -- & 53.0 & 24.4 & 65.6 & \\ 
         & $acc_r$ & 50.0 & 51.2 & 51.6 & 62.1 & 62.2 & 58.6 & 76.7 &  \\
        \midrule
        \multirow{4}{*}{\parbox{17mm}{Counting small numbers}} & $acc$ & 50.0 & -- & -- & -- & 55.4 & 50.6 & 69.2 & \\
         & $p_c$ & 50.0 & -- & -- & -- & 50.0 & 76.6 & 76.7 & \\ 
         & $p_f$ & 50.0 & -- & -- & -- & 60.8 & 24.7 & 61.7 & \\ 
         & $acc_r$ & 50.0 & 48.7 & 49.8	 & 62.5	 & 69.2	 & 62.9	 & 80.2 &  \\
        \midrule
        \multirow{4}{*}{\parbox{17mm}{Counting adversarial}} & $acc$ & 50.0 & -- & -- & -- & 49.9 & 51.8 & 66.7 & \\
         & $p_c$ & 50.0 & -- & -- & -- & 61.5 & 86.1 & 59.5 & \\ 
         & $p_f$ & 50.0 & -- & -- & -- & 37.3 & 17.5 & 74.0 & \\ 
         & $acc_r$ & 50.0 & 69.5 & 45.3 & 57.5 & 42.6 & 73.7 & 77.3 &  \\
        \midrule
        \multirow{4}{*}{\parbox{17mm}{Relations}} & $acc$ & 50.0 & -- & -- & -- & 50.8 & 49.9 & 53.4 & \\
         & $p_c$ & 50.0 & -- & -- & -- & 73.1 & 98.3 & 93.5 & \\ 
         & $p_f$ & 50.0 & -- & -- & -- & 28.4 & 1.5 & 13.3 & \\ 
         & $acc_r$ & 50.0 & 77.2 & 75.0 & 64.3 & 60.2 & 57.2 & 67.7 &  \\
        \midrule
        \multirow{4}{*}{\parbox{17mm}{Action replacement}} & $acc$ & 50.0 & -- & -- & -- & 51.1 & 52.6 & 57.3 & \\
         & $p_c$ & 50.0 & -- & -- & -- & 35.8 & 93.2 & 66.7 & \\ 
         & $p_f$ & 50.0 & -- & -- & -- & 66.4 & 11.9 & 47.8 & \\ 
         & $acc_r$ & 50.0 & 65.4 & 66.8 & 75.6 & 54.8 & 70.7 & 65.9  & \\
        \midrule
        \multirow{4}{*}{Actant swap} & $acc$ & 50.0 & -- & -- & -- & 48.5 & 50.4 & 52.2 & \\
         & $p_c$ & 50.0 & -- & -- & -- & 36.8 & 93.7 & 66.8 & \\ 
         & $p_f$ & 50.0 & -- & -- & -- & 60.2 & 7.1 & 37.6 & \\ 
         & $acc_r$ & 50.0 & 72.2 & 76.9 & 68.6 & 45.8 & 68.3 & 58.9 & \\ 
         \midrule
        \multirow{4}{*}{Coreference} & $acc$ & 50.0 & -- & -- & -- & 49.8 & 50.0 & 54.4 & \\
         & $p_c$ & 50.0 & -- & -- & -- & 81.2 & 98.7 & 92.9 & \\ 
         & $p_f$ & 50.0 & -- & -- & -- & 18.4 & 1.3 & 15.8 & \\ 
         & $acc_r$ & 50.0 & 45.6 & 54.5 & 52.1 & 46.8 & 47.2 & 75.7 & \\
        \midrule
        \multirow{4}{*}{\parbox{17mm}{Coreference hard}} & $acc$ & 50.0 & -- & -- & -- & 49.0 & 50.0 & 54.3 & \\
         & $p_c$ & 50.0 & -- & -- & -- & 80.8 & 98.1 & 95.2 & \\ 
         & $p_f$ & 50.0 & -- & -- & -- & 17.3 & 1.9 & 13.5 & \\ 
         & $acc_r$ & 50.0 & 45.2 & 50.0 & 49.7 & 44.2 & 48.1 & 69.2  &  \\
        \midrule
        \multirow{4}{*}{FOIL it!} & $acc$ & 50.0 & -- & -- & -- & 70.8 & 55.9 & 71.5 & \\
         & $p_c$ & 50.0 & -- & -- & -- & 72.3 & 98.8 & 94.3 & \\ 
         & $p_f$ & 50.0 & -- & -- & -- & 69.3 & 12.9 & 48.8 & \\ 
         & $acc_r$ & 50.0 & 77.5 & 80.7 & 88.8 & 87.1 & 86.9 & 86.9  & \\         
        \bottomrule
    \end{tabular}
    }
    \caption{Results on all \dataset{} instruments and FOIL it!
    % "Excel" sheet for this in comment here:
    % https://docs.google.com/spreadsheets/d/114y6cvNWFoVDiW2By6oldLlEtM2WlS76pVOppHy1eXU/edit#gid=0
    }
    \label{tab:bench_results}
\end{table*}


==> tables/data_statistics.tex <==

\begin{table}[t]
  \small
  \centering
  %\resizebox{\linewidth}{!}{
  \begin{tabular}{llr}
    \toprule
    {\bf Piece} & {\bf Instrument} & {\bf \# Examples} \\
    \midrule
    existence   & existential quantifiers & 534 \\
    \cmidrule{2-3}
    %\rowcolor{gray!15} 
    plurality   & semantic number & 1000 \\
    \cmidrule{2-3}
    \multirow{3}{*}{counting}   & hard & 1000 \\
    %\rowcolor{gray!15} %counting
    & adversarial   & 756  \\
    %counting 
    & small numbers   & 1000  \\
    \cmidrule{2-3}
    %\rowcolor{gray!15} 
    relations   & prepositions & 1000 \\
    \cmidrule{2-3}
    \multirow{2}{*}{action} & replacement   & 779 \\
    %\rowcolor{gray!15} action 
    & actant swap  & 1000  \\
    \cmidrule{2-3}
    \multirow{2}{*}{coreference}   & VisDial train & 916 \\
    %\rowcolor{gray!15}  coreference
    & hard (VisDial valid) & 141 \\
    \bottomrule
  \end{tabular}
  %}
  \caption{Number of data samples per suite in \dataset{}. \lp{TODO: update numbers after MTurk results.}}
  \label{tab:data-statistics}
\end{table}


==> tables/foil_types2.tex <==


\begin{table*}[t]
    \small
    \centering
    
    \begin{tabular}{@{}M{.1\linewidth}M{.12\linewidth}M{.12\linewidth}M{.12\linewidth}M{.12\linewidth}M{.12\linewidth}M{.12\linewidth}@{}}
      \toprule
       & \bf existence & \bf plurality & \bf counting & \bf relations & \bf actions & \bf coreference\\
      \midrule 
      image             &
      \includegraphics[width=\linewidth]{imgs/existence_example_v7w_2361468.jpg}&
      \includegraphics[width=\linewidth]{imgs/coco_plur.png}&
      \includegraphics[width=\linewidth]{imgs/zebras.png} & 
      \includegraphics[width=.7\linewidth]{imgs/coco_rel_small.png} &
      \includegraphics[width=\linewidth]{imgs/shouting_21.jpg} &
      \includegraphics[width=\linewidth]{imgs/coref_example.jpg} \\
      caption &
      \textit{\footnotesize{There are no animals shown.}}&
      \textit{\scriptsize{\gr{A black cat} sitting on a chair at a table with plate of food and coffee.}} &
      \textit{\gr{Two} zebras standing in a field.} &
      \textit{A pan of broccoli \gr{on} a white stove.} &
      \textit{A \gr{man} shouts at a \gr{woman}.} &
      \textit{\scriptsize{Zebra and water buffalo walk along the tall grass. Are they in a zoo? \gr{No}.}}\\
      
      \rowcolor{gray!15} foil   &
      \textit{There are animals shown.}&
      \textit{\scriptsize{\textcolor{red}{Some black cats} sitting on a chair at a table with plate of food and coffee.}}&
      \textit{\textcolor{red}{Three} zebras standing in a field.}&
      \textit{A pan of broccoli \textcolor{red}{close to} a white stove.}&
      \textit{A \textcolor{red}{woman} shouts at a \textcolor{red}{man}.} & 
      \textit{\scriptsize{Zebra and water buffalo walk along the tall grass. Are they in a zoo? \textcolor{red}{Yes}.}} \\
      
      foil gen. method  &      &  NP replacement  &         & SpanBERT / Simple replacement & exchanging action, swapping roles  & \emph{yes} $\leftrightarrow$ \emph{no}\\
     \rowcolor{gray!15} MLM   & \xmark{} & \xmark{}  & \xmark{} & \cmark{} & \cmark{} & \xmark{} \\
      NLI filter        & \xmark{} &  \cmark{}   &   \xmark{}   &  \cmark{} & \cmark{} & \xmark{}\\
     \rowcolor{gray!15}  dataset & Visual7W & MSCOCO & Visual7W & MSCOCO & SWiG  & VisDial v1.0\\
      image src & MSCOCO & MSCOCO & MSCOCO & MSCOCO & SituNet & MSCOCO\\
      \bottomrule
% \hline
    \end{tabular}
    \caption{Overview of \dataset{} \af{instruments/pieces} with image-caption-foil examples per piece, the foil generation method used, whether masked language modelling (MLM) and NLI filtering were applied, and dataset and image sources.}
    \label{tab:phenomena}
\end{table*}

